A First Look at Mobile Intelligence: Architecture, Experimentation and Challenges

Artificial intelligence (AI) technology makes mobile devices become intelligent objects which can learn and act automatically. Although AI will bring great opportunities for mobile applications, little work has focused on the architecture and the interaction with the cloud. In this article, we present three existing architectures of mobile intelligence in detail and introduce its broad application prospects. Furthermore, we conduct a series of experiments to evaluate the performance of the prevalent commercial applications and intelligent frameworks. Our results show that there is a big gap between Quality of Experience (QoE) requirements and the status quo. So far, we have seen only the tip of the iceberg. We pose issues and challenges to advance the area of mobile intelligence and hope to pave the way for the forthcoming.

==> analysis.tex <==
\section{analysis}

==> architecture.tex <==
\section{architecture}
\textbf{Architecture 1: Fully managed deep learning cloud & mobile}\


The mobile application sends an image classification request to the cloud with required data,
and the cloud responds with the prediction result. The details about the training data and
 trained model are secret. We can only use these models through API.


==> biographies.tex <==
Ziyi Wang (wangziyi0821@gmail.com) is now a Ph.D. student in the Department of Computer Science and
Technology, Tsinghua University. His supervisor is Prof. Yong Cui.
His research interests include mobile system and mobile computing.\\

Yong Cui (cuiyong@tsinghua.edu.cn) received his B.E. and Ph.D. degrees in computer science and engineering
from Tsinghua University, China, in 1999 and 2004, respectively.
He is currently a full professor at Tsinghua University and Co-Chair of IETF IPv6 Transition WG Softwire.
His major research interests include mobile wireless Internet and computer network architecture.
Having published more than 100 papers in refereed journals and conferences, he received
the National Award for Technological Invention in 2013, and the Influential Invention Award
of the China Information Industry in both 2012 and 2004. Holding more than 40 patents,
he has authored three Internet standard documents, including RFC 7040 and RFC 5565,
for his proposal on IPv6 transition technologies. He serves at the Editorial Board on
both IEEE TPDS and IEEE TCC.\\

Zeqi Lai (laizq13@mails.tsinghua.edu.cn) is now a Ph.D. student in the Department of Computer Science and
Technology, Tsinghua University. His supervisor is Prof. Yong Cui.
His research interests include cloud computing and cloud storage.


==> insight.tex <==
%\section{insight}
\textbf{1. Existing cloud-based and local-based solutions' latency doesn't meet the real-time interaction demand.\\}

\textbf{2. The DNN model can be split into different kinds of layers, which
are respectively responsible for different functions.\\}

\textbf{3. The distribution of latency varies a lot and is closely related to the corresponding workload.}
DNN has a significant effect on the handling of image and audio, which brings great opportunities in mobile intelligence.
However, for different scenarios, the processing methods adopted are different.
Specifically, image services spend almost all of the execution cycles on DNN computation; speech and NLP services require substantial pre-processing and post-processing, which consume almost half of the execution cycles [7].
Even in the same scenario, if we adopt different model, latency distribution and the corresponding bottleneck are also different.
For example, DeepMon [8] indicates that the convolutional layers dominate the execution cycles in the VGG-VeryDeep-16 and YOLO model.
DeepEye [9] demonstrates that the loading of fully-connected layers is the most time consuming task across 8 different models.
Neurosurgeon [10] indicates that for AlexNet, VGG and DeepFace, convolution layers are most time-consuming; for MNIST, fully-connected layers are most time-consuming; for Kaldi and SENNA, layers of the model incur similar latency.
We can find that the distribution of latency varies a lot and is closely related to the corresponding workload.
In order to make full use of mobile sensor data and cloud computing resources, we should propose a deep integration architecture between mobile and cloud, which splits the functional modules intelligently according to different workload, model, network condition and server load.

